Anonymous Networking amidst Eavesdroppers

The problem of security against timing based traffic analysis in wireless networks is considered in this work. An analytical measure of anonymity in eavesdropped networks is proposed using the information theoretic concept of equivocation. For a physical layer with orthogonal transmitter directed signaling, scheduling and relaying techniques are designed to maximize achievable network performance for any given level of anonymity. The network performance is measured by the achievable relay rates from the sources to destinations under latency and medium access constraints. In particular, analytical results are presented for two scenarios: For a two-hop network with maximum anonymity, achievable rate regions for a general m x 1 relay are characterized when nodes generate independent Poisson transmission schedules. The rate regions are presented for both strict and average delay constraints on traffic flow through the relay. For a multihop network with an arbitrary anonymity requirement, the problem of maximizing the sum-rate of flows (network throughput) is considered. A selective independent scheduling strategy is designed for this purpose, and using the analytical results for the two-hop network, the achievable throughput is characterized as a function of the anonymity level. The throughput-anonymity relation for the proposed strategy is shown to be equivalent to an information theoretic rate-distortion function.

==> required_files/setup.tex <==

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\setcounter{footnote}{1}
%\input /user/ltong/tex/macros/macros.tex
\makeatletter
\newdimen{\captionwidth}
\long\def\@makecaption#1#2{%
\captionwidth 1.0\hsize% use current value of \hsize
\vskip 10pt%
\setbox\@tempboxa\hbox{#1: #2}%
  \ifdim \wd\@tempboxa >\captionwidth%
    \setbox\@tempboxa\hbox{#1:\hspace*{.5em}}%
    \hfil\parbox{\captionwidth}{\raggedright\hangindent \wd\@tempboxa%
    \hangafter=1\unhbox\@tempboxa#2}\hfill%
%  \else \hbox to\captionwidth{\hfil\box\@tempboxa\hfil}%
  \else\centerline{\box\@tempboxa}%
  \fi
}
\makeatother
%\input epsf
\def\scalefig#1{\epsfxsize #1\textwidth}
\makeatletter
\font\hmed=cmr10 at 10pt
\def\ps@plain{\let\@mkboth\@gobbletwo
     \def\@oddhead{}\def\@oddfoot{\hmed\hfil
 / \footernote\ / \qquad \thepage}
\def\@evenhead{}\def\@evenfoot{\hmed
\thepage\qquad /  / \footernote\ \hfil }
}
\def\footernote{{\it \small }} 

\makeatother

\makeatletter
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{A}
\newtheorem{properties}{Properties}
\newtheorem{conjecture}{Conjecture}
\newtheorem{criterion}{Criterion}

%\bibliographystyle{ieee}

\renewcommand\baselinestretch{1.0}

%\footernote{\protect\tiny Submitted to IEEE Transactions On Signal Processing}









